XCC: An X-ray FEL-based $\gamma\gamma$ Compton Collider Higgs Factory

This report describes the conceptual design of a $\gamma\gamma$ Higgs factory in which 62.8 GeV electron beams collide with 1 keV X-ray free electron laser (XFEL) beams to produce colliding beams of 62.5 GeV photons. The Higgs boson production rate is 80,000 Higgs bosons per 10$^7$ second year, roughly the same as the ILC Higgs rate at $\sqrt{s}$=250 GeV. The electron accelerator is based on cold copper distributed coupling (C$^3$) accelerator technology. Unlike the center-of-mass energy spectra of previous optical wavelength $\gamma\gamma$ collider designs, the sharply peaked $\gamma\gamma$ center-of-mass energy spectrum of XCC produces model independent Higgs coupling measurements with precision on par with $e^+e^-$ colliders. For the triple Higgs coupling measurement, the XCC center-of-mass energy can be upgraded to 380 GeV, where the cross section for $\gamma\gamma\rightarrow HH$ is twice that of $e^+e^- \rightarrow ZHH$ at $\sqrt{s}$=500 GeV. Design challenges are discussed, along with the R\&D to address them, including demonstrators.

==> Acknowledgements/Acknowledgments.tex <==

\section{Acknowledgements}

This work was supported in part by the U.S. Department of Energy (DOE) (Contract No. DE-AC02-76SF00515).



==> Synergies_with_Other_Concepts_and_Facilities/Synergies.tex <==

\section{Synergies with other concepts and/or existing facilities}
The XCC would have strong particle physics synergies with LHC.  If  XCC and an $e^+e^-$ collider were both built, there would be clear particle physics synergies between XCC and the $e^+e^-$ collider.  In the nearer term, there are strong synergies between and XCC, C$^3$ and LCLS in the development of the accelerator technology required to realize the XCC or C$^3$-250. 


